A Multilingual Similarity Dataset for News Article Frame

Understanding the writing frame of news articles is vital for addressing social issues, and thus has attracted notable attention in the fields of communication studies. Yet, assessing such news article frames remains a challenge due to the absence of a concrete and unified standard dataset that considers the comprehensive nuances within news content. To address this gap, we introduce an extended version of a large labeled news article dataset with 16,687 new labeled pairs. Leveraging the pairwise comparison of news articles, our method frees the work of manual identification of frame classes in traditional news frame analysis studies. Overall we introduce the most extensive cross-lingual news article similarity dataset available to date with 26,555 labeled news article pairs across 10 languages. Each data point has been meticulously annotated according to a codebook detailing eight critical aspects of news content, under a human-in-the-loop framework. Application examples demonstrate its potential in unearthing country communities within global news coverage, exposing media bias among news outlets, and quantifying the factors related to news creation. We envision that this news similarity dataset will broaden our understanding of the media ecosystem in terms of news coverage of events and perspectives across countries, locations, languages, and other social constructs. By doing so, it can catalyze advancements in social science research and applied methodologies, thereby exerting a profound impact on our society.

==> table-bkups-2024-02-14.tex <==
\begin{table}[tb!]
\begin{center}
\resizebox{0.4\textwidth}{!}{
    \begin{tabular}{cccc}
    \toprule
    Type & Predictor & \makecell{VIF model\\coeeficient} &  \makecell{AIC model\\coeeficient} \\
    \toprule
    
    & {\color{gray} Intercept} & $0.347$ & $0.414$  \\
    \midrule
    
    Pol. & {\color{blue} Federalism?} & $0.118^{**}$  & $0.069^{**}$ \\
    %\hline
    
    %\hline
    & {\color{blue} Within NATO?} & $0.073^{**}$ & $0.044^{**}$ \\
    %\hline
    & {\color{blue} Within EU?} & $-0.028^{**}$ & $-0.093^{*}$   \\
    %\hline
    & {\color{blue} Within BRICS?} & $0.006^{**}$  & $0.012^{**}$   \\
    
    & {\color{blue} Democracy index} &  & $0.175^{**}$  \\
    & {\color{blue} Peace index} &  & $-0.195^{**}$  \\
    
    \midrule
    Soc. & \textbf{{\color{brown} Gini index}} & $\textbf{0.174}^{**}$ & $\textbf{0.196}^{**}$ \\
    %\hline
    
    & {\color{brown} Population} & $0.146^{*}$ & $0.102^{*}$ \\
    %\hline
    & {\color{brown} Net Migration} &  & $0.027^{**}$\\
    %\hline
    
    \midrule
    Geo. & {\color{green} Area} & & $0.093^{**}$\\
    %\hline
    \midrule
    
    Cul. & {\color{purple} \#media} & $-0.148^{**}$ & $-0.130^{**}$    \\
    & {\color{purple} Same media?} & $-0.069^{**}$ & $-0.063^{**}$  \\
    %\hline
    
    & {\color{purple} \#languages} & $0.212^{**}$ & $0.250^{**}$   \\
    %\hline
    & {\color{purple} \#language families} & $0.058^{**}$ & $0.038^{**}$  \\
    & {\color{purple} Religion diversity} & $0.154^{**}$ & $0.126^{**}$ \\
    %\hline
    & {\color{purple} \textbf{Internet user ratio}} & $\textbf{0.300}^{**}$ & $\textbf{0.371}^{**}$ \\
    & {\color{purple} Literacy Ratio} &  & $-0.126^{**}$ \\

    \bottomrule
    \end{tabular}
    }
\caption{News diversity regression coefficients. Positive coefficients mean more news diversity. Predictor color corresponds to its category. The top 2 predictors (according to both the VIF and AIC models) are in bold. Missing predictors or values indicate they are dropped during feature selection process. ** and * symbols stand for 0.005 and 0.01 confidence intervals respectively. }
\label{tab:intra_country_model_result}
\end{center}
\end{table}


\begin{table}[tb!]
\resizebox{1\columnwidth}{!}{
    \centering

    \begin{tabular}{ccccccccc}
    \toprule
    Type & Predictor & \makecell{VIF model\\coefficient} &  \makecell{AIC model\\coefficient} & \\
    \midrule
    & {\color{gray} Intercept} & $0.238$ & $0.247$ \\
    \midrule
    Econ. & {\color{orange} \textbf{Trade}} & $\textbf{0.132}^{*}$& $\textbf{0.155}^{**}$\\
    %\hline
    % & {\color{orange} Same GDP category} & & \\
    % %\hline
    % & {\color{orange} GDP (low--low)} & & \\
    %\hline
    & {\color{orange} GDP (high--high)} & $0.073^{*}$& $0.073^{*}$ \\
    %\hline
    & {\color{orange} GDP (low--high)} & $0.011^{**}$ &   \\
    \midrule
    %\hline
    Pol. & {\color{blue} Same government mode} & $0.010^{*}$& \\
    %\hline
    % & {\color{blue} Both republic} & &  \\
    %\hline
    & {\color{blue} Both federalism} & $0.059^{*}$& $0.057^{**}$\\
    %\hline
    % & {\color{blue} Neither republic nor federalism} & & \\
    %\hline
    % & {\color{blue} Republic and federalism} & & \\
    %\hline
    % & {\color{blue} Republic and other} & & \\
    %\hline
    & {\color{blue} Federalism and other} & $0.010^{*}$&  \\
    %\hline

    % & {\color{blue} Same political bloc} & &  \\
    %\hline
    & {\color{blue} Both in NATO} & $0.051^{*}$& $0.035^{*}$\\
    %\hline
    % & {\color{blue} Both in EU} & & \\
    %\hline
    & {\color{blue} Both in BRICS} & $0.095^{*}$& $0.086^{*}$\\
    %\hline
    
    % & {\color{blue} Across NATO--EU groups} & & \\
    %\hline
    & {\color{blue} Across NATO--BRICS groups} & $0.046^{*}$& $0.060^{*}$\\
    %\hline
    % & {\color{blue} Across EU--BRICS groups} & &  \\
    %\hline
    \midrule
    
    
    Soc. & {\color{brown} Same Gini index category} & $0.020^{*}$& \\
    %\hline
    % & {\color{brown} Gini index (low--low)} &  & \\
    %\hline
    & {\color{brown} Gini index (high--high)} & $-0.037^{*}$& $-0.042^{**}$\\
    %\hline
    & {\color{brown} Gini index (low--high)} & $-0.018^{*}$& \\
    %\hline

    % & {\color{brown} Same Democracy index category} & & \\
    %\hline
    % & {\color{brown} Democracy index (low--low)} & & \\
    %\hline
    & {\color{brown} Democracy index (high--high)} & $0.076^{*}$& $0.068^{**}$\\
    %\hline
    & {\color{brown} Democracy index (low--high)} & $0.023^{*}$& \\
    %\hline
    \midrule
    
    Geo. & {\color{green} Neighbor} & $0.016^{*}$&\\
    & {\color{green} Same Continent} & $0.012^{*}$& $0.022^{**}$\\
    %\hline
    % & {\color{green} Geographic distance} & & \\
    %\hline
    \midrule
    
    Cul. & \textbf{{\color{purple} Same language}} & $\textbf{0.125}^{*}$& $\textbf{0.139}^{**}$\\
    %\hline
    & {\color{purple} Speak English} & $-0.118^{*}$& $-0.130^{*}$\\
    %\hline
    & {\color{purple} Speak German} & $0.014^{*}$&  \\
    %\hline
    % & {\color{purple} Speak Spanish} &  & \\
    %\hline
    % & {\color{purple} Speak Polish} & & \\
    %\hline
    & {\color{purple} Speak French} & $-0.079^{*}$& $-0.084^{*}$\\
    %\hline
    % & {\color{purple} Speak Chinese} & &  \\
    %\hline
    & {\color{purple} Speak Arabic} & $0.026^{*}$&  \\
    %\hline
    % & {\color{purple} Speak Turkish} & & \\
    %\hline
    & {\color{purple} Speak Italian} & $-0.135^{*}$& $-0.125^{*}$\\
    %\hline
    & {\color{purple} Speak Russian} & $-0.036^{*}$&  \\

    \bottomrule
    \end{tabular}
    }
    
    \caption{News synchrony regression coefficients. Positive co-efficients mean more news synchrony between a pair of countries. Predictor color corresponds to its category. The top 2 predictors (according to both the VIF and AIC models) are in bold. Missing predictors and values indicate they are dropped during feature selection process. GDP is binarized as ``high" (\textgreater \$500 billion) and ``low" (\textless \$500 billion). Democracy index  is encoded as ``high" (\textgreater 5) and ``low" (\textless 5).  ** and * symbols stand for 0.005 and 0.01 confidence intervals respectively.}
    \label{tab:inter_country_different_metrics}
\end{table}


==> tables/pub_agreements.tex <==

% Source: https://vw-project.slack.com/archives/C01EJ90U4NQ/p1629312987302600?thread_ts=1629225069.287500&cid=C01EJ90U4NQ
% We need to recompute these numbers using Fabian's script:
% without Chengzhi and Po-Tsun:
% [1] "GEO"
% [1] ":::"
% [1] "GWET:"
% [1] 0.74687
% [1] "Krippendorff:"
% [1] 0.74662
% [1] "-------------------------------------------"
% [1] "ENT"
% [1] ":::"
% [1] "GWET:"
% [1] 0.8298
% [1] "Krippendorff:"
% [1] 0.75577
% [1] "-------------------------------------------"
% [1] "TIME"
% [1] ":::"
% [1] "GWET:"
% [1] 0.77417
% [1] "Krippendorff:"
% [1] 0.38592
% [1] "-------------------------------------------"
% [1] "NAR"
% [1] ":::"
% [1] "GWET:"
% [1] 0.74003
% [1] "Krippendorff:"
% [1] 0.66973
% [1] "-------------------------------------------"
% [1] "OVERALL"
% [1] ":::"
% [1] "GWET:"
% [1] 0.82172
% [1] "Krippendorff:"
% [1] 0.77978
% [1] "-------------------------------------------"
% [1] "TONE"
% [1] ":::"
% [1] "GWET:"
% [1] 0.57229
% [1] "Krippendorff:"
% [1] 0.51547
% [1] "-------------------------------------------"
% [1] "STYLE"
% [1] ":::"
% [1] "GWET:"
% [1] 0.55027
% [1] "Krippendorff:"
% [1] 0.37775
% [1] "-------------------------------------------"


\begin{table}[tb]
    \centering

    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{lrrrrrrr}
    \toprule
     &  GEO &  ENT & TIME  & NAR & OVERALL  \\
    \midrule
Krippen. & 0.73 & 0.69 & 0.57 & 0.69 & 0.77  \\
Gwet & 0.81 & 0.67 & 0.75 & 0.69 & 0.76  \\
    \bottomrule
    \end{tabular}
    }
    
    \caption{Inter-rater agreement measures, Krippendorf's $\alpha$ and Gwet's AC$_{1}$, for each labeled dimension.}
    \label{tab:agreements}
\end{table}


==> tables/pub_annotators_pearson_with_mean.tex <==
\begin{table}[tbh]
    \centering

    \scalebox{0.84}{
    \begin{tabular}{lrrrrr}
    \toprule
    id &  items &  shared & seconds/item  &  correlation \\
    \midrule
    1  &    1,657 &            809 &            296 &     0.88 \\
    2  &    2,311 &            495 &            344 &     0.86 \\
    3  &    1,197 &            611 &            237 &     0.85 \\
    4  &    1,178 &            794 &            213 &     0.85 \\
    5  &     134 &             98 &            153 &     0.84 \\
    6  &    1,036 &            626 &            128 &     0.84 \\
    7  &    1,302 &            345 &            220 &     0.84 \\
    8  &     466 &            398 &            224 &     0.84 \\
    9  &     787 &            208 &            233 &     0.84 \\
    10 &     887 &            368 &            506 &     0.83 \\
    11 &    1,062 &            466 &            387 &     0.82 \\
    12 &     361 &            321 &            311 &     0.81 \\
    13 &     262 &            213 &            165 &     0.81 \\
    14 &     139 &            135 &            235 &     0.79 \\
    15 &    1,076 &            716 &             71 &     0.77 \\
    % 1  &    3300 &           1150 &            262 &     0.88 \\
    % 2  &    1522 &           1006 &            196 &     0.85 \\
    % 3  &    4275 &            633 &            260 &     0.85 \\
    % 4  &    1685 &            850 &            227 &     0.85 \\
    % 5  &     529 &            451 &            216 &     0.85 \\
    % 6  &    1200 &            743 &            121 &     0.84 \\
    % 7  &    1803 &            235 &            178 &     0.84 \\
    % 8  &    1762 &            383 &            189 &     0.83 \\
    % 9  &    1286 &            418 &            506 &     0.82 \\
    % 10 &     508 &            442 &            219 &     0.81 \\
    % 11 &     300 &            258 &            158 &     0.80 \\
    % 12 &    2571 &            795 &            272 &     0.80 \\
    % 13 &     148 &            148 &            230 &     0.78 \\
    % 14 &    1589 &           1094 &             66 &     0.78 \\
    % 15 &     198 &            158 &            106 &     0.73 \\
    \bottomrule
    \end{tabular}
    }
    
    \caption{Annotators and their statistics: the number of labeled items (news article pairs), the number of shared items (also annotated by another annotator), median number of seconds to label an item, and Pearson correlation of their OVERALL labels with the mean labels of other annotators. Only annotators with at least 100 labels are shown.}
    \label{tab:annotators}
\end{table}


==> tables/pub_lang1_pearson_with_mean.tex <==
\begin{table}[tb]
    \centering
    
    \scalebox{0.84}{
    \begin{tabular}{lrr}
    \toprule
    languages &  annotations &  mean(OVERALL) \\
    \midrule
       en &    5,189 &         2.92 \\
       de &    2,166 &         2.56 \\
       es &     955 &         2.40 \\
       zh &     866 &         2.24 \\
     de-en &     863 &         3.20 \\
       tr &     817 &         2.79 \\
       pl &     584 &         2.36 \\
       ar &     572 &         2.41 \\
     es-en &     504 &         2.79 \\
       it &     411 &         2.65 \\
     es-it &     320 &         2.29 \\
       ru &     289 &         2.78 \\
     zh-en &     253 &         3.04 \\
       fr &     184 &         2.39 \\
     de-fr &     116 &         1.88 \\
     pl-en &      77 &         2.38 \\
     de-pl &      35 &         1.69 \\
     fr-pl &      11 &         1.91 \\
    %   en &    6,419 &         2.89 \\
    %   de &    3,251 &         2.56 \\
    %   zh &    2,784 &         2.30 \\
    %   es &    2,238 &         2.35 \\
    %  de-en &    1,949 &         2.94 \\
    %   ar &    1,640 &         2.66 \\
    %   tr &    1,238 &         2.63 \\
    %   it &     803 &         2.64 \\
    %  es-en &     759 &         2.84 \\
    %   pl &     741 &         2.35 \\
    %  zh-en &     523 &         2.97 \\
    %  es-it &     474 &         2.29 \\
    %   ru &     350 &         2.77 \\
    %   fr &     267 &         2.15 \\
    %  de-fr &     178 &         1.92 \\
    %  pl-en &     119 &         2.35 \\
    %  fr-en &      99 &         1.22 \\
    %  fr-pl &      53 &         1.67 \\
    %  de-pl &      47 &         1.69 \\
    \bottomrule
    \end{tabular}
    }
    
    \caption{The number of annotations and the mean OVERALL label (the higher, the more dissimilar) across the 10 languages and their combinations.}
    \label{tab:lang_dist}
\end{table}


